Self-Supervised Pre-training with Combined Datasets for 3D Perception in Autonomous Driving

The significant achievements of pre-trained models leveraging large volumes of data in the field of NLP and 2D vision inspire us to explore the potential of extensive data pre-training for 3D perception in autonomous driving. Toward this goal, this paper proposes to utilize massive unlabeled data from heterogeneous datasets to pre-train 3D perception models. We introduce a self-supervised pre-training framework that learns effective 3D representations from scratch on unlabeled data, combined with a prompt adapter based domain adaptation strategy to reduce dataset bias. The approach significantly improves model performance on downstream tasks such as 3D object detection, BEV segmentation, 3D object tracking, and occupancy prediction, and shows steady performance increase as the training data volume scales up, demonstrating the potential of continually benefit 3D perception models for autonomous driving. We will release the source code to inspire further investigations in the community.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\ynote}[1]{ \color{red} [yanyong: #1]  \color{black}}
\newcommand{\shumin}[1]{\color[rgb]{0,0.6,0}[shumin: #1] \color{black}}
\newcommand{\lnote}[1]{\color{yellow}[lidian: #1] \color{black}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/x_evaluation_backup.tex <==
\section{Evaluation results}
\label{section:eval}
In this section, we will conduct detailed evaluations of our pre-training framework and multi-dataset training approach, and explore how our method leverages large-scale data for pre-training to continually improve the performance of autonomous driving 3D perception models. In summary, we aim to address the following three research questions (RQs):

\textbf{RQ1}: Can our proposed pre-training framework effectively improve model performance on downstream tasks and accelerate model convergence? (Ref section~\ref{section:exp_pretrain_effect})

\textbf{RQ2}: Can the prompt adapter technique we employ help mitigate the domain gap between 3D datasets in a self-supervised pre-training framework? (Ref section~\ref{section:exp_dataset_fusion})

\textbf{RQ3}: Does our proposed approach demonstrate the potential for continuous improvement in performance as the scale of data increases, thereby enabling evolutionary growth? (Ref section~\ref{section:exp_scaling})
\subsection{Effectiveness of pre-training framework}
\label{section:exp_pretrain_effect}
\begin{table*}
    \centering
    \caption{Evaluation of our pre-training framework with baseline methods on downstream tasks. The models are pre-trained on NuScenes dataset and fine-tuned on 20\% of NuScenes dataset. To fit the scope of the paper, we only use the self-supervised loss when reproducing BEVDistill.\shumin{zhuoran finish the pre-train, lidian,zhipeng,liheng do evaluation.}}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
        \multirow{2}*{Pre-training Method}& \multicolumn{2}{c}{3D Object Detection}& \multicolumn{2}{c}{3D Object Tracking} & BEV Segmentation &\multicolumn{2}{c}{Occupancy Prediction}   \\
        \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-6}\cmidrule(r){7-8}
        
        & mAP$\uparrow$&NDS$\uparrow$&AMOTA$\uparrow$&AMOTP$\downarrow$ &mIoU$\uparrow$&mIoU$\uparrow$&IoU$\uparrow$\\
        \midrule
        Scratch & $51.52_{\pm 0.76}$ & $53.47_{\pm 0.51}$ & $57.1_{\pm 0.01}$ & $80.9_{\pm 0.01}$ & $39.17_{\pm 0.39}$ & $15.7_{\pm 0.4}$ & $32.3_{\pm 0.6}$\\
        BEVDistill &$54.06_{\pm 0.01}$ &$57.48_{\pm 0.55}$ & & & $39.06_{\pm 0.10}$ &$15.8_{\pm 0.1}$ &$32.3_{\pm 0.3}$ \\
       % SimIPU & & & & & & & \\
        \rowcolor{gray!20}
        Ours & $53.36_{\pm 0.45}$ & $54.17_{\pm 1.99}$ & $58.7_{\pm 0.01}$ & $77.2_{\pm 0.02}$ & $38.92_{\pm 0.29}$ &$16.0_{\pm 0.4}$ &$32.4_{\pm 0.3}$ \\
        \bottomrule
   
    \end{tabular}}
    
    \label{tab:pretrain_effect}
\end{table*}

We use the NuScenes dataset alone as the pre-training dataset to validate the effectiveness of our multimodal pre-training framework. For comarison, we take two baselines:
\begin{itemize}
    \item Scratch: Randomly initialize the networks without any pre-training.
    \item BEVDistill: State-of-the-art pre-training method that was designed to distill knowledge from pre-trained image network to point cloud network but can also be adopted to train models from scratch~\cite{chen2022bevdistill,sun2023calico}.
\end{itemize}

Table \ref{tab:pretrain_effect} presents a comparison of the performance on various downstream tasks between our method and baseline methods. In the tasks of 3D object detection, 3D object tracking, and occupancy prediction, our pre-training method achieved significant performance improvements. And is more effective when training the models from scratch. To address whether both the losses in our framework contributes to the performance gain, we provide ablation study by removing one of the loss functions. As shown in Table \ref{tab:pretrain_ablation_loss}, both loss functions provides significant benefit to the models' performance in downstream tasks.
\begin{table}
    \centering
    \begin{tabular}{l|cc}
    \toprule
         Pre-training Method& L1 mAP &L1 mAPH  \\
         \midrule 
         Scratch&65.94&61.86\\ 
         BEVDistill&1&1\\ 
         %SimIPU&1&1\\ 
         Ours&66.63&62.57\\ 
         \bottomrule
    \end{tabular}
    \caption{Evaluation on 3D object detection task about the robustness of our pre-training framework when the domain shifts. The models are pre-trained on NuScenes dataset and fine-tuned on 20\% of Waymo dataset.\shumin{zhuoran finish the pre-train, lidian do evaluation.}}
    \label{tab:pretrain_ood}
\end{table}

In addition, we fine-tune the NuScenes-pretrained models on the Waymo dataset for 3D object detection task and test their performance. This will show the robustness of different methods against domain shift. Results in table \ref{tab:pretrain_ood} show that our method also effectively enhances model performance in out-of-distribution scenarios, demonstrating strong generalization capabilities.

\begin{tcolorbox}[colback=gray!10, colframe=black, title=RQ1 Summary:]
Our proprsed pre-training framework can effectively improve models' performance on various downstream tasks with the contribution of all components in both in-domain and out-of-domain scenarios.
\end{tcolorbox}

\begin{table}
    \centering
    \begin{tabular}{l|ccc}
    \toprule
         Loss func& mAP &NDS &mIoU  \\
         \midrule
         Full & $53.3_{\pm 0.5}$ & $54.2_{\pm 2.0}$ & $38.9_{\pm 0.3}$ \\ 
         -$\mathcal{L}_{MAE}$ &$54.1_{\pm 0.9}$ & $58.0_{\pm 0.8}$ & $39.1_{\pm 0.3}$ \\ 
         -$\mathcal{L}_{Contrastive}$ & 1 & 1 & $39.2_{\pm 0.2}$ \\ 
         \bottomrule
    \end{tabular}
    \caption{Ablation study about the contributions of the losses we use in our pre-training framework. The models are evaluated on 3D object detection task.\shumin{zhuoran finish the pre-train, lidian,zhipeng do evaluation.}}
    \label{tab:pretrain_ablation_loss}
\end{table}


\subsection{Multi dataset pre-training}
\label{section:exp_dataset_fusion}
Following to the settings in Section \ref{section:exp_pretrain_effect}, we conduct pre-training under the following configurations: 
\begin{itemize}
    \item  Single dataset: Pre-training using only the NuScenes dataset.
    \item  Multi-dataset w/o prompt: Pre-training with combined datasets by simply mixing the NuScenes, Lyft, and ONCE datasets.
    \item  Multi-dataset w/ prompt: Pre-training with NuScenes, Lyft, and ONCE, utilizing our prompt training strategy.
\end{itemize}

Based on the results in Table \ref{tab:dataset_fusion}, simply mixing the datasets for pre-training do not effectively improve the model's performance on downstream tasks, and even decrease the model's performance on some tasks. However, using the prompt-based multi-dataset training strategy led to a significant performance improvement in all downstream tasks, proving it's effectiveness of mitigating the domain gap between 3D datasets.
\\
\begin{table*}
    \centering
    \begin{tabular}{lccccccc}
    \toprule
        \multirow{2}*{Pre-training Method}& \multicolumn{2}{c}{3D Object Detection}& \multicolumn{2}{c}{3D Object Tracking} & BEV Seg. &\multicolumn{2}{c}{Occupancy Prediction}\\
        \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-6}\cmidrule(r){7-8}
        
        & mAP$\uparrow$&NDS$\uparrow$&AMOTA$\uparrow$&AMOTP$\downarrow$ &mIoU$\uparrow$&mIoU$\uparrow$&IoU$\uparrow$\\
        \midrule
        Single dataset&$53.3_{\pm 0.4}$&$54.2_{\pm 2.0}$&$58.7_{\pm 0.01}$&$77.2_{\pm 0.02}$&$38.9_{\pm 0.3}$&$16.0_{\pm 0.4}$&$32.3_{\pm 0.6}$\\
        Multi-dataset w/o prompt&$52.4_{\pm 0.9}$&$54.5_{\pm 0.6}$&$58.0_{\pm0.01}$&$78.3_{\pm 0.01}$&$39.6_{\pm 0.4}$&$15.9_{\pm 0.1}$&$31.8_{\pm 0.2}$\\
        \rowcolor{gray!20}
        Multi-dataset w/ prompt&$53.5_{\pm 0.2}$&$55.7_{\pm 1.2}$&$59.2_{\pm 0.01}$&$77.4_{\pm 0.00}$&$41.4_{\pm 0.1}$&$16.3_{\pm 0.2}$&$32.7_{\pm 0.1}$\\
        \bottomrule
   
    \end{tabular}
    \caption{Evaluation of models' performance on downstream tasks with different pre-training strategies conducted. NuScenes only represents the model is pre-trained using only NuScenes dataset. The others are pre-trained on the fusion dataset combined with NuScenes, Lyft and ONCE with or without dataset prompt. The evaluation is conducted on NuScenes dataset.\shumin{lehan update evaluation.}}
    \label{tab:dataset_fusion}
\end{table*}

One problem people may concern is that during the pre-training phase, we set different tunable prompts and corresponding adapters for various datasets. However, when applying the pre-trained model to downstream tasks, we do not always use data similar to what was used during pre-training. Thus, the impact of different strategies for using prompts during fine-tuning is crucial. Specifically, when we cannot select an appropriate prompt from those obtained during the pre-training process, is our dataset fusion method still effective?
To address this issue, we conduct experiments with the following strategies during fine-tuning on NuScenes dataset:
\begin{itemize}
    \item Correspond: Initialize the prompt of NuScenes with the correct one obtained from pre-training.
    \item C\&Freeze: Initialize the prompt of NuScenes with the correct one obtained from pre-training and freeze it during fine-tuning.
    \item Wrong: Initialize the prompt of NuScenes with the prompt of another dataset(i.e., ONCE) obtained from pre-training.
    \item Random: Randomly Initialize the prompt of NuScenes with Gaussian distribution.
\end{itemize}
In addition, we take pre-training with combined dataset without prompt training strategy as a baseline. Results in table \ref{tab:effect_prompt} indicates that while initializing with the correct prompt achieves the best downstream performance, using a mismatched prompt still outperforms a naive dataset mixture. This suggests that our method effectively mitigates conflicts between datasets within the backbone network, preserving generalizable knowledge across datasets.
\begin{table}
    \centering
    \begin{tabular}{l|ccc}
    \toprule
        \multirow{2}*{Prompt strategie}& \multicolumn{2}{c}{3D object det.}& BEV seg.\\
        \cmidrule(r){2-3}\cmidrule(r){4-4}
        
        & mAP&NDS&mIoU\\
        \midrule
        w/o prompt & $52.43_{\pm 0.91}$ & $54.53_{\pm 0.60}$ & $39.57_{\pm 0.35}$\\
        Correspond & $53.47_{\pm 0.18}$ & $55.67_{\pm1.15}$ & $41.40_{\pm 0.11}$ \\
        C\&Freeze & $54.29$ & $55.96$ & $41.02_{\pm 0.38}$ \\
        Wrong & & & $41.20_{\pm 0.09}$ \\
        Random & & & $39.08_{\pm 0.14}$ \\
        \bottomrule
   
    \end{tabular}
    \caption{Comparison of different strategies of using prompt during fine-tuning. The evaluations are conducted using NuScenes dataset on 3D object detection and BEV segmentation task.\shumin{lidian,zhipeng do evaluation.}}
    \label{tab:effect_prompt}
\end{table}

\begin{tcolorbox}[colback=gray!10, colframe=black, title=RQ2 Summary:]
The prompt adapter technique we employ can effectively help mitigate the domain gap between 3D datasets in our self-supervised pre-training framework.
\end{tcolorbox}
\subsection{Scalability of the pre-training methods}
\label{section:exp_scaling}
As we stated in Section \ref{section:intro}, the main purpose of our research is to explore expanding the scale of training data to enhance the capabilities of 3D perception models. After validating the effectiveness of our pre-training framework and multi-dataset training method, we further demonstrate that our approach consistently improves model performance as the training data scale increases.

We progressively expanded the sample size from the ONCE dataset from 50,000 to 200,000 and 500,000, while applying repeated sampling on the NuScenes and Lyft datasets to balance the scale differences between datasets (sampling ratios are detailed in Table X). Experimental results in table \ref{tab:dataset_scaling} show that as the training data volume increases, model performance improves significantly across all four downstream tasks, demonstrating that our training method has strong scalability.
\begin{table*}
    \centering
    \caption{Evaluation of models' performance on downstream tasks with different pre-training strategies conducted. NuScenes only represents the model is pre-trained using only NuScenes dataset. The others are pre-trained on the fusion dataset combined with NuScenes, Lyft and ONCE with or without dataset prompt. The evaluation is conducted on NuScenes dataset.\shumin{zhuoran finish the pre-train, lidian,zhipeng,liheng do evaluation.}}
    \begin{tabular}{lccccccc}
    \toprule
        \multirow{2}*{Data Volume}& \multicolumn{2}{c}{3D Object Detection}& \multicolumn{2}{c}{3D Object Tracking} & BEV Segmentation &\multicolumn{2}{c}{Occupancy Prediction}   \\
        \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule(r){6-6}\cmidrule(r){7-8}
        
        & mAP$\uparrow$&NDS$\uparrow$&AMOTA$\uparrow$&AMOTP$\downarrow$ &mIoU$\uparrow$&mIoU$\uparrow$&IoU$\uparrow$\\
        \midrule
        40K Frame&$0$&$0$&$0$&$0$&$0$&&\\
        100K Frame&$53.5_{\pm 0.2}$&$55.7_{\pm 1.2}$&$59.2_{\pm 0.6}$&$77.4_{\pm 0.2}$&$41.4_{\pm 0.1}$&$16.3_{\pm 0.2}$&$32.7_{\pm 0.1}$\\
        250K Frame&$54.1_{\pm 0.6}$&$56.1_{\pm 0.3}$&$59.5_{\pm 0.7}$&$77.1_{\pm 0.7}$&$42.3_{\pm 0.3}$&&\\
        \bottomrule
   
    \end{tabular}
    
    \label{tab:dataset_scaling}
\end{table*}
Results in table~\ref{} indicate that our method achieves performance improvements when using either larger datasets or more datasets.
\begin{tcolorbox}[colback=gray!10, colframe=black, title=RQ3 Summary:]
Our method demonstrates a stable improvement in model performance as the data scale increases, indicating strong scalability and showing potential for building a foundation model for 3D perception with sufficient data.
\end{tcolorbox}

==> sec/x_intro_backup.tex <==
\section{Introduction}
\label{section:intro}


Significant advances have been achieved in model performance through scaling up model sizes, dataset sizes, and computational resources in the field of natural language processing (NLP)~\cite{radford2019language} and 2D computer vision~\cite{dehghani2023scaling}.
We thus use the term \textbf{``scaling effect''}  to refer to the trend that larger models exhibit emergent properties and achieve superior performance when trained on sufficiently large datasets~\cite{kaplan2020scalinglawsneurallanguage}. 
Despite these successes, the field of 3D vision  %, particularly multimodal 3D perception, 
has not yet witnessed the effect of scaling. 
Given the importance of 3D vision, especially for applications such as autonomous driving and robotics, we as a community would like to investigate whether the scaling effect also applies to this area. 

As the first step toward achieving this goal, our paper explores whether 3D vision models could benefit from larger training datasets and if so, by how much.  Specifically, as state-of-the-art 3D vision models on most tasks and benchmarks such as BEVFusion~\cite{liu2023bevfusion}, CMT~\cite{Yan_2023_ICCV_cmt}, SparseLIF~\cite{zhang2024sparselif} and UniTR~\cite{wang2023unitr} are all multimodal models that combine camera images and LiDAR point clouds,  we focus on such LiDAR-camera fusion-based 3D vision models in our work\footnote{In the remainder of the paper, we use 3D vision models, multimodal 3D vision models, LiDAR-camera fusion-based 3D vision models interchangeably unless otherwise specified.}.


To examine whether common 3D vision models can benefit from larger datasets, we first enlarge the popular datasets including  NuScenes~\cite{caesar2020nuscenes}, Lyft~\cite{mandal2021lyft}, ONCE~\cite{mao2021one} by mixing them together and train the models with the mixed datasets. We then evaluate the effect of scaling by measuring the performance of several subsequent tasks including 3D object detection, 3D object tracking, BEV semantic segmentation and occupancy prediction . By taking advantage of existing datasets, we can avoid the prohibitively high costs of collecting, cleaning, and labeling data involved in creating a brand new dataset as in 
~\cite{caesar2020nuscenes,sun2020scalability,mao2021one}.


In the process of enlarging existing datasets, we need to address several technical challenges, among which the most notable are the scarcity of annotation and the domain gap between datasets.
Firstly, we discuss the challenge of annotation scarcity. Many existing 3D vision datasets are usually very small due to the high costs involved in creating a dataset -- e.g., 
%The scarcity of annotation arises because existing annotated 3D vision datasets are often relatively small in scale. For example, widely used annotated datasets like 
NuScenes and Waymo~\cite{sun2020scalability} only contain around one thousand scenes. Meanwhile, larger-scale 3D vision datasets, such as ONCE~\cite{mao2021one} and NuPlan~\cite{caesar2022nuplanclosedloopmlbasedplanning} that contain hundreds of thousands of scenes, are often unannotated (i.e., unlabeled) and cannot be utilized by traditional 3D vision model training methods that rely on 3D annotations. %are unable to leverage these larger-scale datasets. %hindering our research on scaling up the training data.

Thus, a self-supervised training method that can utilize unlabeled datasets is needed. Previous works have explored self-supervised pre-training to %assist in scaling up 3D vision models
leverage unlabeled datasets for 3D vision, but they fall short of our purpose. For example, 
single-modality pre-training methods such as~\cite{chen2020simple,he2019moco,he2021maskedautoencodersscalablevision}, though perform well in single modality tasks, lack cross-modality alignment and may lead to suboptimal results when applied in multi-modality scenes~\cite{}. Multimodal pre-training methods %~\cite{zhou2023unidistilluniversalcrossmodalityknowledge, sautier2022imagetolidarselfsuperviseddistillationautonomous} 
are available but often focus on knowledge distillation from one modality to another, rather than learning from scratch for both modalities. They either consider distilling knowledge from previously pre-trained 2D networks into the point cloud modality~\cite{sautier2022imagetolidarselfsuperviseddistillationautonomous,zhou2023unidistilluniversalcrossmodalityknowledge} or focus on enhancing 3D information in the image modality through point clouds~\cite{liu2023geomim}. However, they do not account for learning unified and efficient feature representations from paired image and point cloud data. This limitation hinders these methods from learning from a large dataset. In this paper, we propose a 3D vision pre-training framework that combines self-supervised pre-training methods for both intra-modalities and inter-modalities, capturing feature representations of images and point clouds while aligning them. Our framework can also be easily expanded to other modalities such as radar, voice and even text. and serve as a universal pre-training framework for 3D vision tasks. %\ynote{I can see the story here. Need to make it flow better.} % explain our architecture more clearly here or later?????????????????????????????

%The success of large NLP and 2D vision models can be likely attributed to the availability of vast amounts of data collected across the internet, which makes self-supervised pre-training and foundational models possible. However, existing multimodal 3D perception datasets are mainly comprised of manually collected sensor data, such as LiDAR point clouds and camera images, whose sizes are seriously limited by the prohibitively high costs involved in data collection~\cite{caesar2020nuscenes,sun2020scalability,mao2021one}. The limited data availability in turn limits 
%the scalability \ynote{scalability or size?} of 3D perception models. To address this challenge, we propose to leverage self-supervised pre-training methods to expand multimodal 3D perception models, thereby reducing dependency on large annotated datasets. As such, this approach enables the models to serve as foundational models that can be fine-tuned for various applications. \ynote{need to revise. What is the takeaway message in this paragraph? Unclear to me.}

Secondly, we discuss how to address the domain gap between datasets. Different datasets have different collection scenes, sensor models, and sensor angles across different 3D vision datasets. 
As a result, When we merge the datasets, training can become unstable and suffer from diverging loss functions. % 
In fact, in 2D and 3D model training, various techniques ~\cite{wu2024towards,kim2022learning,wang2022cross,zhou2022simple} have been developed to address performance degradation due to differences between datasets. Drawing inspiration from these methods\ynote{be specific and say what technique you leverage here}, we devise a prompt adapter to disentangle dataset biases from the backbone network, rendering the model to leverage larger and more diverse data sources more effectively. 

%To scale up our model, larger datasets are crucial ~\cite{kaplan2020scalinglawsneurallanguage}. The limited capacity of single datasets for 3D multimodal perception has significantly hindered the scaling process.
%A direct method to expand the training scale is combining multiple large datasets.
%However, unlike the extensive internet dataset collected for natural language processing and 2D computer vision tasks,
%each 3D multimodal dataset represents a biased sample of the real world, leading to substantial domain gaps (e.g., differences in sensor placement and data collection scenarios). 
%When moving to merged datasets, training can become unstable and the loss diverges, resulting in suboptimal performance. 
%This challenge closely parallels issues encountered in domain adaptation. In traditional 2D and 3D model training, various techniques ~\cite{wu2024towards,kim2022learning,wang2022cross,zhou2022simple} have been developed to address performance degradation across different datasets. Drawing inspiration from these methods, we introduce a prompt adapter designed to disentangle dataset biases from the backbone network, thereby enabling the model to effectively leverage larger and more diverse data sources.

In this paper, we propose a unified framework that leverages self-supervised pre-training methods to asist expand the training dataset of multimodal 3D vision models. Our framework is designed to reduce dependency on large annotated datasets and enhance the data scalability in 3D vision domain.. By integrating multiple popular datasets for pre-training, we scale the training dataset to xxx\shumin{fill the scale of the final dataset}. The results in 3D object detection, 3D object tracking, BEV semantic segmentation, and occupancy prediction demonstrate that through our pre-training method, the performance of 3D vision models exhibits a steady improvement with the increase in training data. % inspiring further research on the scaling law in the field of 3D vision.

To summarize, we make the following contributions: 
\begin{itemize}
    \item We propose a balanced, self-supervised pre-training framework for multimodal 3D vision models
    %, designed to serve as a universal pre-training framework in the 3D domain 
    which can help network of different modalities learn effective and unified feature representations, thereby achieving better performance of multimodal 3D vision tasks.
    
    \item We employ prompt-based domain adaptation techniques to jointly pre-train 3D vision models at a large scale across multiple datasets. Our method can be flexibly applied to different modalities and mitigates the gap between datasets in a unified manner.
    %\item %We conduct a scaling study, increasing the training dataset to xxx \shumin{fill the scale of the final dataset}, and demonstrate that it adheres to predictable scaling trends, resulting in improved 3D vision performance across multiple downstream tasks.
    \item We evaluate our model on four tasks: 3D object detection, BEV semantic segmentation, 3D object tracking, and occupancy prediction. \ynote{summarize our results} %Through our research, we aim to explore the potential of 3D vision models through large-scale pre-training and to inspire further research on general-purpose foundation models in the 3D vision domain.
    We observe that ***, which suggests that *** \ynote{observations}
\end{itemize}






